Disperse-Then-Merge: Pushing the Limits of Instruction Tuning via Alignment Tax Reduction

Supervised fine-tuning (SFT) on instruction-following corpus is a crucial approach toward the alignment of large language models (LLMs). However, the performance of LLMs on standard knowledge and reasoning benchmarks tends to suffer from deterioration at the latter stage of the SFT process, echoing the phenomenon of alignment tax. Through our pilot study, we put a hypothesis that the data biases are probably one cause behind the phenomenon. To address the issue, we introduce a simple disperse-then-merge framework. To be concrete, we disperse the instruction-following data into portions and train multiple sub-models using different data portions. Then we merge multiple models into a single one via model merging techniques. Despite its simplicity, our framework outperforms various sophisticated methods such as data curation and training regularization on a series of standard knowledge and reasoning benchmarks.

==> 1-introduction-v1.tex <==
\section{Introduction}
%paragraph 1
%the question: LLM alignment instruction tuning
Trained on trillions of tokens from webpages on the internet with the next-token prediction objective~\citep{achiam2023gpt4,bai2023qwen,anil2023gemini}, large language models~(LLMs) have demonstrated impressive capacity on obtaining general-purpose representations for various downstream NLP tasks. However, pre-trained language models may not follow human instructions~\citep{ouyang2022training} and even produce toxic, hallucinated or biased content~\citep{sun2024trustllm,huang2023survey,zhang2023sirens}. To address the issue, supervised fine-tuning~\citep{ouyang2022training} on instruction-following data has emerged as one of the \textit{de facto} paradigms for aligning LLMs with human preferences and values. 
Recently, a surge of models tuned on massive high-quality instruction-following data such as  Alpaca~\citep{taori2023alpaca} and Vicuna~\citep{chiang2023vicuna}  have verified the effectiveness of supervised fine-tuning.

% paragraph 2

% problem: the cost of alignment: alignment tax; 
% As the no-free-launch theorem~\citep{} goes, the alignment of LLM may not work well for all problems and also incur a potential side effect. Actually, previous research has noticed the ``alignment tax'', which refers to the phenomenon that after an LLM is aligned with human intent and preference, its performance on traditional NLP benchmark might decline. Recently, \citept{} also observed that the performance of Llama-2 degrades on knowledge-intensive benchmarks after it goes through SFT process and attributed the performance drop to the interference to the parametric knowledge by the instruction data, since there exist incorrect or irrelevant answers in the instruction data collected from strong GPT-4 teacher~\citep{}.   
% how to object this? 
% however, we find that large language models are not sui



% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figure/tulu-7b-updown.pdf}
%     \caption{The performance on MMLU (5-shot, accuracy) and BBH (3-shot, exact match) after tuning Llama-2-7b with different numbers of \tulu-V2-mix instruction data.}
%     \label{fig:tulu-7b-updown}
% \end{figure}

\begin{figure}
\centering
\begin{subfigure}{0.45\linewidth}
\includegraphics[width=\linewidth]{figure/tulu-mmlu-updown.pdf}
\caption{The performance on MMLU (5-shot, accuracy) v.s. data size.}
\label{fig:tulu-mmlu-updown}
\end{subfigure}
\begin{subfigure}{0.45\linewidth}
\includegraphics[width=\linewidth]{figure/tulu-bbh-updown.pdf}
\caption{The performance on BBH (3-shot, exact match) v.s. data size.}
\label{fig:tulu-bbh-updown}
\end{subfigure}
\caption{The performance on MMLU and BBH when tuning Llama-2-7b and Llama-2-13b with different sizes of instruction-following data from \tulu-V2-mix.}
\label{fig:tulu-updown}
\end{figure}


%However, a recent study~\citep{} discovers that the instruction-following ability of LLM does not always improve with the data size growing but saturates early if the instruction is of high quality. 

However, with the size of instruction-following data rising, it has been observed that the performance of LLM on conventional knowledge and reasoning benchmarks does not always improve or even exhibits degradation~\citep{dou2023loramoe}, echoing the alignment tax phenomenon in \citet{bai2022training}. As shown in Figure~\ref{fig:tulu-updown}, when tuning Llama-2-7b~\citep{touvron2023llama2} on \tulu-V2-mix~\citep{ivison2023camels}, as we gradually increase the instruction-following data size, the accuracy on MMLU~\citep{hendrycks2021mmlu} and BBH~\citep{suzgun2023bbh} first rises up to reach a peak and degrades afterward. In other words, simply scaling up the instruction-following data leads to a quick bump into the upper bound where the marginal return of increasing data size approaches zero or minus. It is therefore a non-trivial challenge to unleash the full potential of large-scale instruction-following data.




%Putting together, simply scaling up the instruction data leads to a quick bump into the upper bound with the marginal return of more data approaching zero or becoming minus. It is therefore non-trivial to unleash the full potential of large-scale instruction data.
%Consequently, the performance on instruction direct fine-tuning on large-scale instruction data is probably not the best choice for 


% parapraph3 
% pilot study observation: 1. alignment tax does not happen at start, but go through a up-down process. 2. the loss on train set decrease faster than test;



% However, through our pilot study~(Section~\ref{}) on various LLMs and instruction corpora, we discover that even on sophisticated constructed instruction data (e.g. tulu~\citep{}), the alignment tax still exists, indicating that the alignment tax is probably not caused by low-quality cases in the instruction data. 


% Prior literature~\citep{dou2023loramoe} tends to attribute the problem to the interference to the parametric knowledge of LLM caused by the low-quality instruction data~\citep{chen2023alpagasus,cao2023instruction}. 
Prior literature~\citep{chen2023alpagasus,cao2023instruction} tends to attribute the problem to the low-quality samples within the instruction-following corpus, which are over-fitted by the LLM and lead to the interference to the parametric knowledge.  However, as observed in our pilot study (Section~\ref{sec:pilot}), the performance drop even happens when tuning on meticulously curated high-quality data like \tulu-V2-mix~\citep{ivison2023camels}. Alternatively, by analyzing the trend of loss descending on the training set and validation set, we hypothesize that the alignment tax is caused by the data bias acquired by LLM. Specifically, during the SFT process, LLMs not only learn the generalizable instruction-following capacities but also tend to exploit dataset biases as shortcuts for predictions. The learning speed of the latter gradually outpaces the former, eventually resulting in a decline in conventional knowledge and reasoning benchmarks when the harm of dataset biases outweighs the benefit of generalizable instruction-following capacities. 


% but also simultaneously assimilate the data-specific biases that are incapable of generalizing to standard benchmark~\citep{du2021towards,wang2022identifying}. When the assimilated bias assumes a dominant role, the performance of the model experiences a decline. 





% 1) The metric on standard NLP benchmarks does not fall precipitously from the beginning, but goes through a rise-fall during the instruction tuning process. And more importantly, 2) Even on sophisticated constructed instruction data (e.g. tulu~\citep{}), the rise-fall trend also appears, suggesting that the alignment tax is not depends on the data quality.







% hypothesis: the reason of alignment tax is data bias
% A hypothesis~\citep{} for the reason of this phenomenon is the forgetting of parametric knowledge stored in
% LLMs during the fine-tuning process since the decline on knowledge-insensitive benchmarks is observed to be much more acute than that on other benchmarks. To take a further step, we investigate the difference between the pre-training data and instruction data in terms of embodied world knowledge. As shown in the Figure~\ref{}, it is discovered that the world knowledge within the instruction data is \textit{scare} in quantity and \textit{long-tailed} in distribution when compared with the pre-training data. As a result, the distribution mismatch of world knowledge may interfere with the parametric knowledge acquired from the pre-training stage, thus putting a limit on the scaling effect of instruction data



% paragraph 4 
% our approach: split then merge
% To break , \citept{} propose LoRAMoE architecture to partition different capabilities within distinct sections of LoRA~\citep{} in a mixture-of-expert~\citep{} manner which requires an alteration in model architecture and introduces extra parameters. Meanwhile, \citept{} put forward another intuitive solution involving choosing the most valuable estimated by a proxy function, leaving a significant portion of data abandoned. Different from previous works, we aim at a lightweight and portable solution to maximize the potential of full instruction data. 
As a possible remedy for the problem, we propose a frustratingly simple \modelname~(\textbf{D}isperse-\textbf{T}hen-\textbf{M}erge) framework composed of three steps: (1) we initially distribute the instruction-following data into several clusters and then (2) perform instruction tuning on each cluster of data to obtain a series of sub-models assimilating different data biases; (3) finally we merge the sub-models trained on each cluster into a single one in the weight space, such that the data bias of each sub-model is mitigated in the fused one. %In summary, we distribute dataset biases into a set of sub-models and eliminate them through the merging of sub-models. 
Consequently, \modelname ensures the reduction of alignment tax when instruction tuning with almost no extra cost at training and inference. 
%our framework can lead to a strong instruction-following model while maintaining the capacity on standard benchmarks.  




%we get inspiration from~\citep{}, which reports that merging two models possessing different shortcuts will result in a shortcut-free model as the unique shortcut of each model is forgotten at merging. 


% paragraph 5
% experiment result
To empirically verify the efficacy of the \modelname\ framework, we conduct extensive experiments on Llama-2-7b and other LLMs. Evaluations across $9$ benchmarks involving math reasoning, world knowledge, and code generation indicate that \modelname outperforms a variety of meticulously designed and intricate instruction tuning methods such as LoRAMoE~\citep{dou2023loramoe} and Deita~\citep{liu2023what}. In particular, \modelname generally achieves an absolute improvement of  $0.5\sim1.5$ on MMLU~\citep{hendrycks2021mmlu} and BBH~\citep{suzgun2023bbh} compared with vanilla SFT.   


The contribution of this paper can be summarized as follows:
\begin{itemize}[wide=0.\parindent,noitemsep,topsep=0.em]
    \item We empirically verify and analyze the effect of alignment tax during the instruction tuning, thereby putting a hypothesis that the dataset biases are the reason behind the alignment tax.
    \item We propose a frustratingly easy \modelname framework in which the biases from instruction-following data are distributed and forgotten.
    % \item Together, our exploration presents another piece of the broader puzzle of understanding the LLM alignment.
\end{itemize}
 
 
 






% paragraph 6 
% sum up contribution 





==> response.tex <==
Response To Metareview

We are grateful for the expertise and efforts of all reviewers and area chairs in reviewing our work. We are encouraged and excited by the recognition of the simplicity and efficacy of our proposed framework.

Q1: More analysis and details to support the proposed hypothesis.
A1: In the final version, we would definitely follow the advice of area chairs and elucidate on more details about our analysis of alignment tax. Specifically, following the advice of the reviewers, we delved deeper into our experiment in Section 3 to inspect the alignment tax from a fine-grained token-level perspective. By measuring the correlation between the per-token loss reduction on the training set and the validation set, we discovered that the fitting on the training set tokens is less likely to improve generalization ability on the validation set as the tuning process goes on, which further supports our hypothesis. 


Q2: More analysis regarding the number of clusters and different merging methods
A2: Thanks for your suggestions!  we would move the supplementary experiment results in Appendix B.2 into the main document with extra space.







General Response

We extend our deepest gratitude for the insightful feedback and valuable suggestions provided. Furthermore, we are excited to receive the acknowledgment of the strengths in our work, notably:

+ In-depth analysis of the alignment tax phenomenon and the data bias hypothesis as a possible reason behind it. (Reviewer dZDk)
+ Introduction of a novel framework called Disperse-Then-Merge (DTM) and interesting empirical study on using it to address alignment tax. (Reviewer uC2v and AF1S)
+ Extensive experiments and insightful analysis to support the proposed approach. (Reviewer dZDk, uC2v and AF1S)

We sincerely thank you again for your invaluable suggestions, which mainly focus on the ambiguity of experiment implementation details. We would definitely incorporate your advice and move Appendix A.2 into our main document. Should there be any further concerns or questions, we are fully prepared and eager to address them.






Dear Reviewer AF1S,

Thank you again for your valuable time to review our work and constructive feedback. We posted our response to your comments approximately two days ago, and we wonder if you could kindly share some of your thoughts so we can keep the discussion rolling to address your concerns if there are any.

In the previous response,

1. We make a further illustration of the details of our experiment setting, including the rationale of in-context example numbers, the motivation for employing LoRA in our main experiment, and the core idea of our pilot study. We are sorry for the ambiguity and we would definitely complement the details in the main document.     
2. We perform a significant test on our main experiment and the results show that our approach exceeds the vanilla SFT on a variety of knowledge and reasoning benchmarks, suggesting the efficacy of our approach in mitigating the alignment tax with almost no extra cost at both the training stage and the inference stage.
3. We further explore the impact of the data size on experimental performance, which answers the question concerning the application scenario of our approach. 

We would appreciate it if you could kindly take a look at our response to your comments. If you have any further questions, we are happy to discuss them!

Best regards,

All authors of Paper4688




Dear Reviewer dZDK,

Thank you again for your valuable time to review our work and constructive feedback. We posted our response to your comments approximately two days ago, and we wonder if you could kindly share some of your thoughts so we can keep the discussion rolling to address your concerns if there are any.

In the previous response,

1. We further illustrate our implementation details on the first step of our framework and delineate the robustness of the data dispersal step.     
2. We release a sample of our code in an anonymous Github repository, and we plan to release a more detailed version of our code together with our checkpoint upon publishing.


We would appreciate it if you could kindly take a look at our response to your comments. If you have any further questions, we are happy to discuss them!

Best regards,

All authors of Paper4688


Response to Reviewer uC2v:

Thanks for your time and expertise in reviewing our work! We are excited to receive your recognition that our work is insightful and sound, which is a great encouragement to us. In below We would like to address your concerns one by one:

Question1: The LoRA fine-tuning configuration is not clear until the limitation section.

Answer1: Thanks for your suggestion! 

We are sorry for the ambiguity in implementation details and the unnecessary misunderstanding it incurs. We would definitely move the experiment details in Appendix A.3 into the main document and describe our experiment configuration more clearly in the final version. 

We primarily perform experiments with LoRA as it is widely adopted as a common practice in SFT[2] and it attains similar performance to full-parameter fine-tuning while requiring fewer computation resources. Therefore, we believe employing LoRA for experiments would not incur losses in generalization, following previous work in SFT[1][2][3]. 

[1]Sun, Zhiqing, et al. "Principle-driven self-alignment of language models from scratch with minimal human supervision." Advances in Neural Information Processing Systems 36 (2024)

[2]Xu, Canwen, et al. "Baize: An Open-Source Chat Model with Parameter-Efficient Tuning on Self-Chat Data." Proceedings of the 2023 Conference on Empirical Methods in Natural Language Processing. 2023.

[3]Lee, Ariel, Cole Hunter, and Nataniel Ruiz. "Platypus: Quick, Cheap, and Powerful Refinement of LLMs." NeurIPS 2023 Workshop on Instruction Tuning and Instruction Following. 2023.



Question2: The caption of Figure 1 and the typos.

Answer2: Thanks for your suggestions! We would definitely follow your advice, adjusting the caption layout and correcting the typos in the final version. 


Response to Reviewer dZDk:

We are grateful for your time and efforts in reviewing our work and we are grateful to receive your praise for our clear motivation and in-depth analysis. We carefully read through your insightful suggestions and we would like to address your concerns one by one: 

Question1: Will the possible errors in the data distribution step affect the subsequent procedures and the overall performance?
 

Answer1: Thanks for your question! Actually, in the main experiment, we adopt the random dispersal of data since other more sophisticated encoding methods do not have an apparent advantage, as shown in Table 2. Besides, we report the average performance of multiple random seeds, Therefore, our data dispersal step is relatively robust and unlikely to incur cascaded errors. 


Question2: The paper should consider open source code.

Answer2: We totally agree that opensourcing source code is significant for the reproducibility of our work so we create an anonymous Github repo containing a sample code: https://anonymous.4open.science/r/ExpertFusion-8B32. We promise to release the code upon publication with a detailed README file to facilitate relevant research in the future. 



Question3: Limited exploration of the impact of data clustering and model fusion methods.

Answer3: Thanks for your suggestion! We analyze the effect of different data clustering methods and different model merging methods in Section 5.2, comparing $6$ more schemes for clustering in Table 2. Specifically, we use MiniLM and MPNet to encode the instruction (I), the response (R) or both of them (I+R) to obtain their dense representation for K-means clustering. Besides, in Table 4, we explore the effect of $5$ widely-used merging techniques (average merge, fisher merge, task vector merge, tie merge and DARE). Reviewer uC2v also agrees that our analysis of these sophisticated variants is thorough and convincing. We will definitely describe this part more clearly in the final version. Let us know if you have any specific suggestions on what clustering and merging methods should be added. We are more than happy to conduct such experiments.




Response to Reviewer AF1S:

We appreciate your time and effort in reviewing our work! Many thanks for your constructive and valuable feedback, which would definitely make our work better and we would like to address your concerns one by one as follows:

Question1: No experiments on other PEFT techniques such as adapter or full-parameter fine-tuning.

Answer1: Thanks for your suggestion! We mainly perform experiments on LoRA as LoRA is one of the widely adopted PEFT techniques in SFT for its less computation requirement and similar performance to full-parameter fine-tuning. Meanwhile, considering the extensive experiments on large-scale language models, full-parameter fine-tuning is computationally expensive and probably beyond the budgets of many academic institutes. Therefore, following previous works[1][2][3] that only use LoRA for SFT, we believe our experiment configuration would not incur much losses in generalization. 

[1]Sun, Zhiqing, et al. "Principle-driven self-alignment of language models from scratch with minimal human supervision." Advances in Neural Information Processing Systems 36 (2024)

[2]Xu, Canwen, et al. "Baize: An Open-Source Chat Model with Parameter-Efficient Tuning on Self-Chat Data." Proceedings of the 2023 Conference on Empirical Methods in Natural Language Processing. 2023.

[3]Lee, Ariel, Cole Hunter, and Nataniel Ruiz. "Platypus: Quick, Cheap, and Powerful Refinement of LLMs." NeurIPS 2023 Workshop on Instruction Tuning and Instruction Following. 2023.



Question2: The improvement against the vanilla fine-tuning baseline seems not significant.

Answer2: Thanks for your advice! We supplement the significant test result in the Table below: 

|            | GSM8K | MMLU  | BBH   | ARC-c | OBQA | RACE  | Humaneval | MBPP | TruthfulQA |
|------------|-------|-------|-------|-------|------|-------|-----------|------|------------|
| Vanilla    | 18.50  | 49.74 | 42.78 | 46.93 | 32.80 | 40.57 | 17.68     | 21.40 | 25.83  |
| DTM (Ours) | 20.62* | 50.43*| 44.46*| 48.72* | 33.80 | 41.34* | 18.29 | 23.60*| 29.13*|

Where $^*$ denotes significant improvement over the vanilla SFT (t-test, $p< 0.05$).

From the table, we can observe that our approach outperforms vanilla SFT significantly on most world knowledge and commonsense reasoning benchmarks. Notably, the evaluation benchmarks used in our experiment are highly comprehensive and challenging (e.g., MMLU contains $57$ sub-tasks and BBH contains $27$ sub-tasks) such that gigantic improvement is rather difficult or even unrealistic, considering that our approach (1) involves no new data and (2) incurs no extra cost at both the training stage and the inference stage. 

Question3: In what scenario is DTM better used? 

Answer3: That is a good question! To explore when our advantage against vanilla SFT is more obvious, we experiment with different sizes of instruction-following data sampled from Tulu-V2-mix and compare our proposed DTM with vanilla SFT. The gap in their performance on BBH (3-shot, measured in exact match) is shown in the Table below:


|  Data Size  | 64k   | 128k  | 192k  | 256k  | 320k  |
|-------------|-------|-------|-------|-------|-------|
| Vanilla SFT | 42.07 | 42.83 | 42.94 | 43.09 | 42.78 |
| DTM (Ours)  | 41.66 | 42.55 | 42.89 | 43.43 | 44.46 |
| Difference  | -0.41 | -0.28 | -0.05 | 0.34  | 1.68  |

From the table, we can observe that DTM has a more obvious advantage at large data size, echoing our previous finding in the pilot study that fitting on data biases is more severe with large data size.

Question4: How to quickly determine the number $K$ of sub-models?

Answer4: It is a good question! The number of sub-models $K$ is a hyper-parameter and we analyze its impact to model performance in Appendix B.2, from which we can see that $K=4$ is probably a good starting point and our approach is relatively insensitive to the choice of $K$ within a specific range. 

Question5: Is the pilot experiment fair? Different amounts of data will have different training steps.   


Answer5: 
Thanks for your question! In the pilot study, we focus on alignment tax, a phenomenon in which LLM performance on standard knowledge and reasoning benchmarks as the size of instruction-following data grows. To perform an in-depth analysis,  we run multiple SFT training varying the instruction-following data size ($20\%, 40\%, 60\%, 80\%,  100\%$) while maintaining the batch size, training epoch number, learning rate schedule and other hyper-parameters unchanged. 

As a result, to draw a fair comparison before different runs, we must adjust the training step accordingly to maintain a constant batch size and constant number of training epochs. Otherwise, pursuing constant training steps suggests adjusting the number of training epochs accordingly (e.g., $1$ epoch for $100\%$ data, $2$ epochs for $50\%$ data, and $5$ epochs for $20\%$ data). Repetitive training on small-scale data may lead to severe overfit and influence our observation. 

Question6: Why are different numbers of in-context examples (shot) set for different tasks at evaluation?

Answer6: Good question! Our evaluation configuration for each task mainly follows precedent work[4][5] and public benchmarks[6] such that our readers can draw a direct comparison. We will put this point more conspicuous in our final version. 

[4]Jiang, Albert Q., et al. "Mistral 7B." arXiv preprint arXiv:2310.06825 (2023).

[5]Ivison, Hamish, et al. "Camels in a changing climate: Enhancing lm adaptation with tulu 2." arXiv preprint arXiv:2311.10702 (2023).

[6]https://huggingface.co/spaces/HuggingFaceH4/open_llm_leaderboard

==> table/main-mmlu.tex <==

\begin{tabular}{lccccc}
\toprule
             & Humanities & \makecell[c]{Social\\ Science} & STEM  & Other & Overall \\
\midrule
Llama-2-base & 43.30      & 51.80          & 37.00  & 52.53 & 45.96   \\
\midrule
Vanilla        & \underline{47.29}      & 56.68          & 39.73 & 56.05 & 49.74   \\
L2-norm           & 46.21      & \underline{57.43}          & \underline{39.86} & \textbf{57.80} & 49.98   \\
EWC          & 45.95      & 56.09          & 38.10 & 56.91 & 49.02   \\
Replay     & 46.16      & 56.13          & 38.97 & \underline{57.68} & 49.46   \\
Uniform Soup         & 47.21      & 57.36          & \textbf{40.29} & 57.13 & \underline{50.24}   \\
MoE          & 44.06      & 54.27          & 37.77 & 54.50 & 47.36   \\
Deita        & 45.57      & 55.48          & 38.40 & 55.55 & 48.50   \\
\midrule
\modelname\ (Ours)         & \textbf{47.52}      & \textbf{58.27}          & 39.23 & 57.62 & \textbf{50.43}   \\
\bottomrule
\end{tabular}
